Which priors matter? Benchmarking models for learning latent dynamics

Learning dynamics is at the heart of many important applications of machine learning (ML), such as robotics and autonomous driving. In these settings, ML algorithms typically need to reason about a physical system using high dimensional observations, such as images, without access to the underlying state. Recently, several methods have proposed to integrate priors from classical mechanics into ML models to address the challenge of physical reasoning from images. In this work, we take a sober look at the current capabilities of these models. To this end, we introduce a suite consisting of 17 datasets with visual observations based on physical systems exhibiting a wide range of dynamics. We conduct a thorough and detailed comparison of the major classes of physically inspired methods alongside several strong baselines. While models that incorporate physical priors can often learn latent spaces with desirable properties, our results demonstrate that these methods fail to significantly improve upon standard techniques. Nonetheless, we find that the use of continuous and time-reversible dynamics benefits models of all classes.

==> results/big_table_results.tex <==
\begin{table*}[t]
\vspace{-10pt}
\begin{center}
\begin{tiny}
\setlength\tabcolsep{3.7pt}
% \begin{tabular}{l|c|cc||cc|c||cc|c||cc|c||cc|c}
\begin{tabular}{l|cc|cc||cc|cc||cc|cc||cc|c||cc|c}
\toprule

Dataset & \multicolumn{4}{c||}{HGN} & \multicolumn{4}{c||}{LGN} & \multicolumn{4}{c||}{Neural ODE} & \multicolumn{3}{c||}{RGN} & \multicolumn{3}{c}{AR} \\
 & Rec & Extrap & Fwd & Bck  & Rec & Extrap & Fwd & Bck  & Rec & Extrap & Fwd & Bck & Rec & Extrap & Fwd & Rec & Extrap & Fwd \\
\midrule
Mass-spring & \textbf{0.05} & \textbf{0.07} & \textbf{1.0} & \textbf{1.0} & 0.06 & 0.13 & \textbf{1.0} & \textbf{1.0} & 0.17 & 0.24 & \textbf{1.0} & 0.91 & 0.18 & 0.25 & \textbf{1.0} & 0.35 & 0.51 & 0.2 \\
Mass-spring +c & \textbf{1.11} & 2.28 & 0.52 & \textbf{0.39} & 3255.2 & 3255.2 & 0.0 & 0.0 & 1.16 & \textbf{2.19} & 0.52 & 0.0 & 1.52 & 2.81 & \textbf{0.56} & 123.0 & 209.82 & 0.07 \\
Mass-spring +c +f & \textbf{1.0} & 2.91 & 0.41 & \textbf{0.13} & 3433.24 & 3433.25 & 0.0 & 0.0 & 1.2 & \textbf{1.67} & \textbf{0.98} & 0.0 & 1.23 & 1.75 & 0.94 & 159.51 & 159.34 & 0.15 \\
Pendulum & \textbf{1.97} & 27.35 & 0.11 & 0.03 & 2.53 & 41.99 & 0.12 & 0.12 & 2.78 & \textbf{13.0} & \textbf{0.45} & \textbf{0.56} & 2.33 & 50.99 & 0.13 & 151.71 & 383.27 & 0.0 \\
Pendulum +c & 25.85 & 104.83 & 0.08 & 0.01 & 34.97 & 105.5 & 0.07 & 0.07 & 29.46 & 76.68 & \textbf{0.12} & \textbf{0.1} & \textbf{23.08} & \textbf{66.77} & 0.1 & 240.88 & 390.78 & 0.0 \\
Pendulum +c +f & \textbf{14.27} & 106.1 & 0.13 & 0.03 & 22.15 & 61.11 & 0.12 & 0.26 & 15.09 & \textbf{37.03} & \textbf{0.3} & \textbf{0.35} & 15.99 & 44.87 & 0.19 & 255.36 & 390.77 & 0.0 \\
Double pendulum & 27.39 & 175.64 & 0.13 & 0.01 & 33.94 & 139.15 & 0.18 & \textbf{0.15} & 20.88 & 111.95 & \textbf{0.2} & \textbf{0.15} & \textbf{19.4} & \textbf{105.92} & 0.19 & 228.03 & 386.67 & 0.0 \\
Double pendulum +c & 100.15 & 100.16 & 0.15 & 0.15 & 60.93 & 87.18 & 0.11 & 0.01 & \textbf{54.61} & \textbf{85.23} & \textbf{0.16} & \textbf{0.26} & 100.15 & 100.15 & 0.15 & 100.16 & 100.16 & 0.15 \\
Double pendulum +c +f & 22.57 & 44.54 & 0.11 & 0.04 & 28.48 & 50.25 & 0.1 & 0.39 & \textbf{21.95} & \textbf{40.22} & 0.17 & \textbf{0.42} & 25.55 & 43.7 & \textbf{0.18} & 99.93 & 527.19 & 0.01 \\
Two-body & \textbf{0.21} & 18.0 & 0.29 & 0.02 & \textbf{0.21} & 3.21 & 0.47 & 0.49 & 0.25 & 0.74 & \textbf{0.99} & \textbf{0.94} & 0.28 & \textbf{0.59} & 0.98 & 0.46 & 3.0 & 0.69 \\
Two-body +c & 10.64 & 49.03 & 0.21 & 0.06 & 2.29 & 24.96 & 0.23 & 0.35 & 2.3 & 15.28 & \textbf{0.24} & \textbf{0.51} & \textbf{1.86} & \textbf{15.24} & \textbf{0.24} & 29.35 & 128.58 & 0.15 \\
3D room - spiral & 106.81 & 286.43 & 0.04 & 0.0 & 2558.07 & 2567.61 & 0.0 & 0.0 & 64.3 & 69.46 & \textbf{0.46} & \textbf{0.45} & \textbf{47.23} & \textbf{57.62} & 0.4 & 1004.83 & 1003.47 & 0.0 \\
3D room - circle & 121.84 & 151.06 & 0.07 & 0.0 & 2823.36 & 2823.35 & 0.0 & 0.0 & 87.37 & 91.04 & 0.35 & \textbf{0.34} & \textbf{65.35} & \textbf{72.19} & \textbf{0.38} & 309.47 & 803.05 & 0.0 \\
MD - 4 particles & 55.5 & 219.52 & 0.18 & 0.01 & 53.2 & 177.09 & 0.21 & 0.06 & 28.41 & \textbf{134.13} & 0.26 & \textbf{0.28} & \textbf{21.93} & 144.22 & \textbf{0.3} & 342.88 & 500.96 & 0.04 \\
MD - 16 particles & 380.63 & 459.35 & 0.0 & \textbf{0.0} & 529.74 & 555.31 & 0.0 & \textbf{0.0} & \textbf{199.89} & \textbf{372.45} & 0.0 & \textbf{0.0} & 580.16 & 580.18 & 0.0 & 524.78 & 800.18 & \textbf{0.01} \\
Matching pennies & \textbf{2.09} & 12.18 & \textbf{0.85} & \textbf{0.86} & 4.32 & 19.43 & 0.53 & 0.61 & 2.22 & \textbf{11.57} & 0.76 & 0.83 & 3.65 & 23.02 & 0.55 & 28.07 & 116.65 & 0.2 \\
Rock-paper-scissors & \textbf{5.13} & 223.96 & 0.1 & 0.01 & 3255.2 & 3255.2 & 0.0 & 0.0 & 5.77 & \textbf{37.11} & \textbf{0.35} & \textbf{0.36} & 5.67 & 37.97 & 0.24 & 8.08 & 99.11 & 0.04 \\
\midrule
% Average & 51.6 & 116.67 & 0.26 & 0.16 & 946.93 & 976.47 & 0.18 & 0.21 & 31.64 & 64.71 & 0.43 & 0.38 & 53.86 & 79.31 & 0.38 & 212.17 & 353.15 & 0.1 \\
% \midrule
Average Rank & \textbf{2.0} & 3.12 & 2.82 & 2.18 & 3.71 & 3.65 & 3.29 & 2.06 & 2.24 & \textbf{1.47} & \textbf{1.65} & \textbf{1.18} & 2.47 & 2.24 & 2.0 & 4.59 & 4.53 & 3.71 \\


\bottomrule
\end{tabular}
\caption{Reconstruction MSE, extrapolation MSE (both $\times10^{7}$), forward (Fwd) and backward (Bck) VPT scores for models with the best average VPT score per model class. VPT scores are presented in proportion to the maximal available dataset rollout length. 
}
\label{tbl_l2_results}
\end{tiny}
\end{center}
\vspace{-12pt}
\end{table*}


==> results/hyper_table_results.tex <==
% \begin{table}[!ht]
% \begin{center}
% \begin{tiny}
% \begin{tabular}{l|l|c}
% \toprule
% Model class & Hyperparameter & Number of datasets best \\
% \midrule
% % \multirow{3}{*}{AR} & GRU & 0.29 \\
% %  & LSTM & 0.53 \\
% %  & Vanilla & 0.18 \\
% %  \midrule
% % HGN & fwd & 1.0 \\
% % \midrule
% % \multirow{2}{*}{LGN} & fwd & 0.47 \\
% %  & fwd/bck & 0.53 \\
% %  \midrule
% % \multirow{4}{*}{ODE} & Direct Diff - fwd & 0.18 \\
% %  & Adjoint - fwd & 0.0 \\
% %  & Direct Diff - fwd/bck & 0.41 \\
% %  & Adjoint - fwd/bck & 0.41 \\
% %  \midrule
% % \multirow{2}{*}{RGN} & Standard & 0.18 \\
% %  & Residual & 0.82 \\
%  \multirow{3}{*}{AR} & GRU & 5 \\
%  & LSTM & 9 \\
%  & Vanilla & 3 \\
%  \midrule
% HGN & fwd & 17 \\
% \midrule
% \multirow{2}{*}{LGN} & fwd & 8 \\
%  & fwd/bck & 9 \\
%  \midrule
% \multirow{4}{*}{ODE} & Direct Diff - fwd & 3 \\
%  & Adjoint - fwd & 0 \\
%  & Direct Diff - fwd/bck & 7 \\
%  & Adjoint - fwd/bck & 7 \\
%  \midrule
% \multirow{2}{*}{RGN} & Standard & 3 \\
%  & Residual & 14 \\
% \bottomrule
% \end{tabular}
% \caption{For each model class we show the number of datasets for which a particular hyperparameter setting ended up with the best model.}
% \vspace{-20pt}
% \label{tbl_stability}
% \end{tiny}
% \end{center}
% \end{table}




\begin{wraptable}{r}{3.5cm}
\vspace{-20pt}
\begin{center}
\begin{tiny}
\begin{tabular}{l|l|c}
\toprule
Model & Hyperp. & N \\
\midrule
% \multirow{3}{*}{AR} & GRU & 0.29 \\
%  & LSTM & 0.53 \\
%  & Vanilla & 0.18 \\
%  \midrule
% HGN & fwd & 1.0 \\
% \midrule
% \multirow{2}{*}{LGN} & fwd & 0.47 \\
%  & fwd/bck & 0.53 \\
%  \midrule
% \multirow{4}{*}{ODE} & Direct Diff - fwd & 0.18 \\
%  & Adjoint - fwd & 0.0 \\
%  & Direct Diff - fwd/bck & 0.41 \\
%  & Adjoint - fwd/bck & 0.41 \\
%  \midrule
% \multirow{2}{*}{RGN} & Standard & 0.18 \\
%  & Residual & 0.82 \\
 \multirow{3}{*}{AR} & GRU & 5 \\
 & LSTM & 9 \\
 & Vanilla & 3 \\
 \midrule
HGN & fwd & 17 \\
\midrule
\multirow{2}{*}{LGN} & fwd & 8 \\
 & fwd/bck & 9 \\
 \midrule
\multirow{4}{*}{N. ODE} & RK2 - fwd & 3 \\
 & Adjoint - fwd & 0 \\
 & RK2 - fwd/bck & 7 \\
 & Adjoint - fwd/bck & 7 \\
 \midrule
\multirow{2}{*}{RGN} & Standard & 3 \\
 & Residual & 14 \\
\bottomrule
\end{tabular}
\caption{Number of datasets for which a particular hyperparameter setting ended up with the best model.}
\vspace{-10pt}
\label{tbl_stability}
\end{tiny}
\end{center}
\end{wraptable}


==> results/std_table_results.tex <==
\vspace{-10pt}
\begin{table}[t]
\begin{center}
\begin{tiny}
\setlength\tabcolsep{3.8pt}
\begin{tabular}{l|cc|cc|cc|c|c}
\toprule

Dataset & \multicolumn{2}{c}{HGN} & \multicolumn{2}{|c}{LGN} & \multicolumn{2}{|c}{Neural ODE} & \multicolumn{1}{|c}{RGN} & \multicolumn{1}{|c}{AR} \\
 & Fwd & Bck & Fwd & Bck  & Fwd & Bck &  Fwd &  Fwd \\
\midrule
Mass-spring & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & 0.2 & \textbf{0.0} & 0.4 \\
Mass-spring +c & \textbf{0.18} & \textbf{0.24} & N/A & N/A & 0.23 & N/A & 0.21 & 0.22 \\
Mass-spring +c +f & 0.17 & \textbf{0.05} & N/A & N/A & \textbf{0.08} & N/A & 0.11 & 0.36 \\
Pendulum & \textbf{0.02} & \textbf{0.01} & 0.05 & 0.03 & 0.32 & 0.26 & 0.03 & N/A \\
Pendulum +c & \textbf{0.03} & N/A & 0.04 & \textbf{0.03} & 0.08 & 0.05 & 0.06 & N/A \\
Pendulum +c +f & \textbf{0.06} & \textbf{0.02} & 0.09 & 0.09 & 0.33 & 0.16 & 0.18 & N/A \\
Double pendulum & \textbf{0.04} & N/A & 0.08 & \textbf{0.07} & 0.13 & 0.08 & 0.1 & N/A \\
Double pendulum +c & 0.36 & 0.36 & \textbf{0.09} & N/A & 0.22 & \textbf{0.32} & 0.36 & 0.36 \\
Double pendulum +c +f & \textbf{0.09} & \textbf{0.02} & 0.1 & 0.09 & 0.18 & 0.15 & 0.27 & N/A \\
Two-body & \textbf{0.03} & N/A & 0.21 & 0.21 & 0.05 & \textbf{0.13} & 0.08 & 0.18 \\
Two-body +c & \textbf{0.05} & \textbf{0.04} & 0.09 & 0.08 & 0.1 & 0.2 & 0.1 & 0.09 \\
3D room - spiral & N/A & N/A & N/A & N/A & 0.46 & \textbf{0.47} & \textbf{0.27} & N/A \\
3D room - circle & \textbf{0.14} & N/A & N/A & N/A & 0.43 & \textbf{0.43} & 0.37 & N/A \\
MD - 4 particles & 0.07 & N/A & 0.13 & \textbf{0.04} & 0.11 & 0.11 & 0.1 & \textbf{0.01} \\
MD - 16 particles & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A \\
Matching pennies & \textbf{0.25} & 0.25 & 0.29 & 0.35 & 0.28 & \textbf{0.24} & 0.34 & 0.4 \\
Rock-paper-scissors & \textbf{0.01} & \textbf{0.0} & N/A & N/A & 0.19 & 0.27 & 0.17 & 0.1 \\
\midrule
Total & \textbf{0.10} & \textbf{0.10} & \textbf{0.10} & \textbf{0.10} & 0.20 & 0.22 & 0.17 & 0.23   \\


% Dataset & \multicolumn{2}{|c||}{HGN} & \multicolumn{2}{|c||}{LGN} & \multicolumn{2}{|c||}{ODE} & \multicolumn{1}{|c||}{RGN} & \multicolumn{1}{|c}{AR} \\
%  & Fwd & Bck & Fwd & Bck  & Fwd & Bck &  Fwd &  Fwd \\
% \midrule
% Mass-spring & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & 0.2 & \textbf{0.0} & 0.4 \\
% Mass-spring +c & \textbf{0.18} & \textbf{0.24} & N/A & N/A & 0.23 & N/A & 0.21 & 0.22 \\
% Mass-spring +c +f & 0.17 & \textbf{0.05} & N/A & N/A & \textbf{0.08} & N/A & 0.11 & 0.36 \\
% Pendulum & \textbf{0.02} & \textbf{0.01} & 0.05 & 0.03 & 0.32 & 0.26 & 0.03 & N/A \\
% Pendulum +c & \textbf{0.03} & N/A & 0.04 & \textbf{0.03} & 0.08 & 0.05 & 0.06 & N/A \\
% Pendulum +c +f & \textbf{0.06} & \textbf{0.02} & 0.09 & 0.09 & 0.33 & 0.16 & 0.18 & N/A \\
% Double pendulum & \textbf{0.04} & N/A & 0.08 & \textbf{0.07} & 0.13 & 0.08 & 0.1 & N/A \\
% Double pendulum +c & 0.36 & 0.36 & \textbf{0.09} & N/A & 0.22 & \textbf{0.32} & 0.36 & 0.36 \\
% Double pendulum +c +f & \textbf{0.09} & \textbf{0.02} & 0.1 & 0.09 & 0.18 & 0.15 & 0.27 & N/A \\
% Two-body & \textbf{0.03} & N/A & 0.21 & 0.21 & 0.05 & \textbf{0.13} & 0.08 & 0.18 \\
% Two-body +c & \textbf{0.05} & \textbf{0.04} & 0.09 & 0.08 & 0.1 & 0.2 & 0.1 & 0.09 \\
% 3D room - spiral & N/A & N/A & N/A & N/A & 0.46 & \textbf{0.47} & \textbf{0.27} & N/A \\
% 3D room - circle & \textbf{0.14} & N/A & N/A & N/A & 0.43 & \textbf{0.43} & 0.37 & N/A \\
% MD - 4 particles & 0.07 & N/A & 0.13 & \textbf{0.04} & 0.11 & 0.11 & 0.1 & \textbf{0.01} \\
% MD - 16 particles & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A \\
% Matching pennies & \textbf{0.25} & 0.25 & 0.29 & 0.35 & 0.28 & \textbf{0.24} & 0.34 & 0.4 \\
% Rock-paper-scissors & \textbf{0.01} & \textbf{0.0} & N/A & N/A & 0.19 & 0.27 & 0.17 & 0.1 \\
% \midrule
% Total & 0.10 & 0.10 & 0.10 & 0.10 & 0.20 & 0.22 & 0.17 & 0.23   \\

\bottomrule
\end{tabular}
\caption{Standard deviations of the forward (Fwd) and backward (Bck) VPT score  for models shown in Table~\ref{tbl_l2_results}. N/A means that the model did not extrapolate well for the dataset.
}
\label{tbl_divergence_var}
\end{tiny}
\end{center}
\vspace{-25pt}
\end{table}

